Application of troubled-cells to finite volume methods -- an optimality study using a novel monotonicity parameter

We adapt a troubled-cell indicator from discontinuous Galerkin (DG) methods to finite volume methods (FVM) with MUSCL reconstruction and using a novel monotonicity parameter show there is a trade-off between convergence and quality of the solution. Employing two dimensional compressible Euler equations for flows with oblique shocks, this trade-off is studied by varying the number of troubled-cells systematically. An oblique shock is characterized primarily by the upstream Mach number, the shock angle $\beta$, and the deflection angle $\theta$. We study these factors and their combinations and find that the degree of the shock misalignment with the grid determines the optimal number of troubled-cells. On each side of the shock, the optimal set consists of three troubled-cells for aligned shocks, and the troubled-cells identified by tracing the shock and four lines parallel to it, separated by the grid spacing, for nonaligned shocks. We show that the adapted troubled-cell indicator identifies a set of cells that is close to and contains the optimal set of cells for a threshold constant $K = 0.05$, and consequently, produces a solution close to that obtained by limiting everywhere, but with improved convergence.

==> 2-Methodology/TestCases/Ramp/Ramp.tex <==
Test Case 4: Flow Over A Ramp. The computational domain for this test case is $[0, 1] \times [0, 1]$ and is divided into $200 \times 200$ cells. A detailed illustration of this test case setup is presented in Figure (\ref{fig:Ramp_setup}). We compute this problem for an inlet Mach number of 3 with ramp angles of \ang{20} and \ang{30}. Supersonic inlet and outlet boundary conditions are applied along the edges AD and BC, respectively and solid slip wall boundary conditions are applied along the edges AB and DC. \\ \\


==> 2-Methodology/TestCases/UnSteadyTestCase.tex <==
\input{./2-Methodology/TestCases/Riemann/Riemann.tex}
\input{./2-Methodology/TestCases/DMR/DMR.tex}

\begin{figure}
\centering
\subfloat[2D Riemann: Configuration 3]{\includestandalone[width=0.4\textwidth]{./2-Methodology/TestCases/Riemann/Config3_setup} \label{fig:config3_setup}}
\subfloat[2D Riemann: Configuration 4]{\includestandalone[width=0.4\textwidth]{./2-Methodology/TestCases/Riemann/Config4_setup} \label{fig:config4_setup}} \\
\subfloat[Double Mach reflection]{\includestandalone[width=0.5\textwidth]{./2-Methodology/TestCases/DMR/DMR_setup2}\label{fig:DMR_setup}}
\caption{Solution domain and initial conditions for unsteady test cases (not drawn to scale).}
\label{fig:Unsteady_setup}
\end{figure}


==> 6-Results/AlignOS/AlignOS.tex <==
\subsection{Aligned Oblique Shock}

% \input{./4-Main/Label_TC_Methods/Align/AlignedShocks.tex}

We solve the two-dimensional Euler equations (\ref{eq:2d_euler}) for the test setup shown in Figure (\ref{fig:AlignOS_setup}), for the first case considering three different shock angles for a given upstream Mach number. The computational domain is initialised with the exact solution corresponding to a upstream Mach number of $3$ and the shock angle of interest. The limiter is applied only to troubled-cells for various configurations given in Table (\ref{tab:TC_CaseNotation_align}).

Density profiles of the cells just above the line $y = 0.5$ for three different oblique shock angles using the medium grid are shown in Figure (\ref{fig:AOS_density_PreAndPost1}) for configurations with a single troubled-cell either in pre- or post-shock region. When limiting is applied only to a single troubled-cell in the pre-shock region, the solution exhibits undershoots in the pre-shock region regardless of the number troubled-cells in the post-shock region. Similarly, when the limiting is applied only to a  single troubled-cell in the post-shock region, the solution exhibits overshoots in the post-shock region regardless of the number troubled-cells in the pre-shock region. This observation is valid for all the three shock angles, although there is a difference in the magnitude of the overshoots or undershoots.

Density profiles of the cells along the same line are shown in Figure (\ref{fig:AOS_density_2and3}) for the remaining configurations `22', `32', `23', and `33'. There are no significant overshoots or undershoots in the solutions of these configurations, although slight overshoots are present for smaller shock angles, especially for configurations with two troubled-cells in the post-shock region.  Across all these configurations, the solutions are quite similar and closely match the solution of limiting everywhere. Notably, configurations `22' and `32' yield identical solutions, as do configurations `23' and `33' for shock angles of \ang{40} and \ang{50}.

\begin{figure}[H]
\centering
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/A30_density_pre1}\label{fig:A30_density_pre1}}
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/A30_density_post1}\label{fig:A30_density_post1}}\\
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/A40_density_pre1}\label{fig:A40_density_pre1}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/A40_density_post1}\label{fig:A40_density_post1}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/A50_density_pre1}\label{fig:A50_density_pre1}}
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/A50_density_post1}\label{fig:A50_density_post1}}
\caption{Aligned oblique shock with inlet Mach 3. Density profiles along the line $y = 0.5$ for three different shock angles on the medium grid. Top row (a, b): \ang{30}. Middle row (c, d): \ang{40}. Bottom row (e, f): \ang{50}. Left column (a, c, e): configurations with a single troubled-cell in the pre-shock. Right column (b, d, f): configurations with a single troubled-cell in the post-shock.}
\label{fig:AOS_density_PreAndPost1}
\end{figure}

\begin{figure}[H]
\centering
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/A30_density_2and3}\label{fig:A30_density_2and3}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/A40_density_2and3}\label{fig:A40_density_2and3}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/A50_density_2and3}\label{fig:A50_density_2and3}}
\caption{Aligned oblique shock with inlet Mach 3. Density profiles along the line $y = 0.5$ for three different shock angles on the medium grid for the configurations `22', `32', `23', and `33'.}
\label{fig:AOS_density_2and3}
\end{figure}

Figure (\ref{fig:AOS_SameMach_TvLinfDiff}) further validates these observations by showing the differences ($\mu$) between the total variation and $L_{\infty}$ norm of the error in density for three different shock angles across all configurations, including the limiting-everywhere case.

For configurations with a single troubled-cell in the pre-shock region, the difference ($\mu$) is significantly higher compared to other configurations, indicating the presence of significant oscillations in the solution. The same holds for configurations with a single troubled-cell in the post-shock region, although the difference ($\mu$) is smaller compared to the configurations with a single troubled-cell in the pre-shock region.

For all other configurations, with at least two troubled-cells in both the pre- and post-shock regions, the difference ($\mu$) is almost of the same order as the limiting everywhere for a particular shock angle, which is of the order $10 ^{-2}$ or smaller. This indicates that the solution for these configurations exhibits fewer oscillations and closely match with the solution obtained from the limiting everywhere approach.

\begin{figure}[H]
\centering
\includestandalone[width=0.25\textwidth]{./4-Main/AlignOS/M3/SameMach/legend}\\[-5ex]
\includegraphics[width=\textwidth]{./4-Main/AlignOS/M3/SameMach/Density}\label{fig:SameMachDensity}
\caption{Aligned oblique shock: $\mu$ for three different shock angles across all configurations, including the limiting-everywhere case. ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:AOS_SameMach_TvLinfDiff}
\end{figure}

From Figure (\ref{fig:AOS_SameMach_TvLinfDiff}), we can also observe that from configuration `22' to `32' (similarly `23' to `33'), the difference is slightly reduced for a shock angle of \ang{30}. However, for shock angles \ang{40} and \ang{50}, it remains exactly the same. This indicates that adding an extra layer of troubled-cells in the pre-shock region is beneficial only for smaller shock angles for a given upstream Mach number. Conversely, from configuration `22' to `23' (similarly `32' to `33'), the difference slightly increases for a shock angle of \ang{30}. However, for shock angles \ang{40} and \ang{50}, it slightly reduces. This suggests that adding an extra layer of troubled cells in the post-shock region is beneficial for higher shock angles (i.e., smaller downstream flow angles), but not for smaller shock angles (i.e., higher downstream flow angles). As the shock angle increases, the relative difference between the total variation and the $L_{\infty}$ norm decreases, indicating that the solver's ability to capture the shock is much better for higher shock angles for a given Mach number.

From here on, we present the results only for configurations with at least two troubled cells both in the pre- and post-shock regions for all other test cases involving aligned shocks. The convergence history of the residual norm $RN$ (Eq. \ref{eq:RN}) versus number of iterations is plotted in Figure (\ref{fig:AlignedOS_M3_RN_Main}) for three different oblique shock angles and configurations `22', `23', `32', and `23'. It can be observed that the solution fully converges (i.e., $RN < 10^{-14}$) to steady-state solution in nearly the same number of timesteps for all these configurations, which is significantly better than the limiting everywhere approach. As the shock angle increases for a given upstream Mach number, the number of iterations required for the residual norm to converge to machine zero also increases.

\begin{figure}[H]
\centering
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/residuenorm_30}\label{fig:AOS_RN_30}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/residuenorm_40}\label{fig:AOS_RN_40}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/residuenorm_50}\label{fig:AOS_RN_50}}
\caption{Aligned oblique shock with inlet Mach 3. The convergence history of the residual norm as a function of number of iterations for configurations `22', `23', `32', and `33', and for limiting everywhere case.}
\label{fig:AlignedOS_M3_RN_Main}
\end{figure}

% For the second case, we varied the Mach numbers for a given shock angle. We selected upstream Mach numbers based on the pressure ratios of previous test cases, i.e., the pressure ratios of an upstream Mach number of 3 and shock angles \ang{30}, \ang{40}, and \ang{50}. For a shock angle of \ang{30}, we chose two other upstream Mach numbers such that the pressure ratio of a shock angle of \ang{30} and one of the chosen upstream Mach numbers matches the pressure ratio of Mach 3 and shock angle of \ang{40}, while the pressure ratio of a shock angle of \ang{30} and the other chosen upstream Mach number matches the pressure ratio of Mach 3 and a shock angle of \ang{50}. Similarly, we selected the upstream Mach numbers for the other two shock angles. Table (\ref{tab:AOS_SameAngle}) presents various Mach numbers for a given shock angle and the corresponding pressure ratios across the shock.

For the second case, we varied the Mach numbers for a given shock angle. We selected upstream Mach numbers based on the pressure ratios of previous test cases, i.e., the pressure ratios of an upstream Mach number of 3 and shock angles \ang{30}, \ang{40}, and \ang{50}. For an upstream Mach number of 3, the pressure ratio across the shock depends on the shock angle. For \ang{30}, it is 2.45833333; for \ang{40}, it is 4.17168040; and for \ang{50}, it is 5.99498626. Now, for the \ang{30} shock angle, we determine upstream Mach numbers so as to get pressure ratios of 4.17168040 and 5.99498626. Similarly for \ang{40} and \ang{50} shock angles. For clarity, the shock angles, Mach numbers, and the corresponding pressure ratios are shown in Table (\ref{tab:AOS_SameAngle}).


\begin{table}[H]
\centering
\caption{For a given shock angle, different Mach numbers and the pressure ratios across the shock for that combination.}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{c c c}
\toprule
Shock Angle & Mach Number & Pressure Ratio ($P_2/P_1$) \\
\midrule
\multirow{3}{*}{\ang{30}} & $M_{PR_1}$ = 3 & $PR_1$ = 2.45833333\\
& $M_{PR_2}$ = 3.85672566 & $PR_2$ = 4.17168040 \\
& $M_{PR_3}$ = 4.59626666 & $PR_3$ = 5.99498626 \\
\midrule
\multirow{3}{*}{\ang{40}} & $M_{PR_1}$ = 2.33358574 & $PR_1$ = 2.45833333\\
& $M_{PR_2}$ = 3 & $PR_2$ = 4.17168040 \\
& $M_{PR_3}$ = 3.57526078 & $PR_3$ = 5.99498626 \\
\midrule
\multirow{3}{*}{\ang{50}} & $M_{PR_1}$ = 1.958110935 & $PR_1$ = 2.45833333 \\
& $M_{PR_2}$ = 2.517298895 & $PR_2$ = 4.17168040 \\
& $M_{PR_3}$ = 3 & $PR_3$ = 5.99498626 \\
\bottomrule
\end{tabular}%
% }
\label{tab:AOS_SameAngle}
\end{table}

\begin{figure}[H]
\centering
\includestandalone[width=0.3\textwidth]{./4-Main/AlignOS/M3/SameAngle/legend}\\[-5ex]
\subfloat[\ang{30}]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignOS/M3/SameAngle/Density2_30}\label{fig:SameAngleDensity_30}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignOS/M3/SameAngle/Density2_40}\label{fig:SameAngleDensity_40}}\\[-2ex]
\subfloat[\ang{50}]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignOS/M3/SameAngle/Density2_50}\label{fig:SameAngleDensity_50}}
\caption{Aligned oblique shock: $\mu$ for three different upstream Mach numbers for a given shock angle. For upstream Mach numbers $M_{PR_1}$, $M_{PR_2}$, and $M_{PR_3}$ (in ascending order), refer Table (\ref{tab:AOS_SameAngle}). ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:AOS_SameAngle_TvLinfDiff}
\end{figure}

Figure (\ref{fig:AOS_SameAngle_TvLinfDiff}) presents the difference between the total variation and $L_{\infty}$ norm of error in density for configurations `22', `32', `23', and `33' for three different upstream Mach numbers for a given shock angle. Previously, we observed that adding an extra layer of troubled-cells in the pre-shock region improved the solution for a \ang{30} shock angle (Figure (\ref{fig:AOS_SameMach_TvLinfDiff})). However, Figure (\ref{fig:SameAngleDensity_30}) indicates that the difference values for configurations `22' and `32' (similarly `23' and `33') are exactly the same as the upstream Mach number increases (i.e., pressure ratio increases). This suggests that adding an extra layer of troubled-cells in the pre-shock region does not affect the solution at all as the upstream Mach number increases (i.e., pressure ratio increases) even for smaller shock angles.

We also observed that adding an extra layer of troubled-cells in the post-shock region slightly improved the solution for \ang{40} and \ang{50} shock angles (Figure (\ref{fig:AOS_SameMach_TvLinfDiff})). However, Figure (\ref{fig:SameAngleDensity_40}) indicates that for \ang{40} shock angle, as the upstream Mach number increases (i.e., downstream flow angle increases), the difference value slightly increases from configuration `22' to `23' (similarly `32' to `33), making the solution worse than the solution with fewer troubled cells in the post-shock region.

Considering the pressure ratio across the shock, the data in Table (\ref{tab:AOS_SameAngle}) can be rearranged with respect to the pressure ratio. For a given  pressure ratio, there are three different combinations of upstream Mach number and shock angles. Figure (\ref{fig:AOS_SamePR_TvLinfDiff}) presents the difference between the total variation and $L_{\infty}$ norm of error in density for configurations `22', `32', `23', and `33' for three different upstream Mach number and shock angle combinations for a given pressure ratio. From this figure, it is observed that for a given pressure ratio, the difference between the total variation and the $L_{\infty}$ norm decreases as the shock angles increases (i.e., the upstream Mach number decreases). This indicates that for a given pressure ratio, solver's ability to capture the shock is better for higher shock angles (i.e., smaller upstream Mach numbers).

\begin{figure}[H]
\centering
\includestandalone[width=0.3\textwidth]{./4-Main/AlignOS/M3/SamePR/legend}\\[-5ex]
\subfloat[$PR_1$]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignOS/M3/SamePR/Density2_PR1}\label{fig:SamePRDensity_PR1}}
\subfloat[$PR_2$]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignOS/M3/SamePR/Density2_PR2}\label{fig:SamePRDensity_PR2}}\\[-2ex]
\subfloat[$PR_3$]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignOS/M3/SamePR/Density2_PR3}\label{fig:SamePRDensity_PR3}}
\caption{Aligned oblique shock: $\mu$ for three different upstream Mach number and shock angle combinations for a given pressure ratio. For pressure ratios $PR_1$, $PR_2$, and $PR_3$ (in ascending order), refer Table (\ref{tab:AOS_SameAngle}). ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:AOS_SamePR_TvLinfDiff}
\end{figure}

\begin{figure}[H]
\centering
\includestandalone[width=0.8\textwidth]{./4-Main/AlignOS/M3/SameAngle/legend_RN}
\includestandalone[width=0.7\textwidth]{./4-Main/AlignOS/M3/SameAngle/legend_RN2}\\
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/SameAngle/RNorm_30}\label{fig:AOS_SameAngle_RN30}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/SameAngle/RNorm_40}\label{fig:AOS_SameAngle_RN40}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/SameAngle/RNorm_50}\label{fig:AOS_SameAngle_RN50}}
\caption{Aligned oblique shock. The convergence history of the residual norm as a function of number of iterations for configuration `23' and for limiting everywhere case, considering three different upstream Mach numbers for a given shock angle. For the upstream Mach numbers $M_{PR_1}$, $M_{PR_2}$, and $M_{PR_3}$, refer Table (\ref{tab:AOS_SameAngle}).}
\label{fig:AOS_SameAngle_RN}
\end{figure}

\begin{figure}[H]
\centering
\includestandalone[width=0.8\textwidth]{./4-Main/AlignOS/M3/SamePR/legend_RN}
\includestandalone[width=0.7\textwidth]{./4-Main/AlignOS/M3/SamePR/legend_RN2}\\
\subfloat[$PR_1$]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/SamePR/RNorm_245}\label{fig:AOS_SamePR_RN245}}
\subfloat[$PR_2$]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/SamePR/RNorm_417}\label{fig:AOS_SamePR_RN417}}\\
\subfloat[$PR_3$]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignOS/M3/SamePR/RNorm_599}\label{fig:AOS_SamePR_RN599}}
\caption{Aligned oblique shock. The convergence history of the residual norm as a function of number of iterations for configuration `23' and for limiting everywhere case, considering three different upstream Mach number and shock angle combinations for a given pressure ratio. For the pressure ratios ($PR$), refer Table (\ref{tab:AOS_SameAngle}).}
\label{fig:AOS_SamePR_RN}
\end{figure}

Figure (\ref{fig:AOS_SameAngle_RN}) presents the convergence history of the residual norm versus the number of iterations for configuration `23' and the limiting everywhere case, considering three different upstream Mach numbers for a given shock angle. Conversely, the Figure (\ref{fig:AOS_SamePR_RN}) presents the same data for three different shock angles for a given pressure ratio. From the first figure, it is observed that convergence to steady-state is achieved in fewer number of iterations as the upstream Mach number increases for a given shock angle. The second figure demonstrates that as the shock angle increases for a given pressure ratio, the number of iterations required for convergence to steady-state also increases.

Overall, for the aligned shocks, the number of troubled cells in the pre-shock region depends on the pressure ratio across the shock as the pressure ratio increases fewer number of troubled cells are sufficient in the pre-shock region. In the post-shock region, it depends on the downstream flow angle with respect to the grid as the downstream flow angle increases fewer number of troubled cells are sufficient in the post-shock region. Convergence to steady-state is significantly improved by limiting only fewer number of troubled-cells compared to limiting everywhere approach.


==> 6-Results/AlignedRamp/AlignedRamp.tex <==
\subsection{Flow over a ramp with an aligned shock}

% Next, we test the case where all three, incoming flow, out flow and the shock , are aligned to the grid. For this we choose a flow over a ramp test case and to get all the three mentioned earlier aligned to the grid computational domain as shown in Figure (\ref{fig:AlignedRamp_setup}). This computational domain consists of two parallelograms ABEF and BCDE. The parallelogram ABEF is constructed such a way that sides AB and EF are parallel to x-axis and sides BE and AF are at an angle $\beta$ (shock angle) to the positive x-axis. The parallelogram BCDE is constructed such a way that sides BC and DE are at an angle $\theta$ (turn angle) to the positive x-axis and the side CD is parallel to the side BE. For different shock angle and turn angle combination, different computational domain is generated.
%
% The computational domain is initialised with an exact solution of respective inlet Mach number, shock angle and turn angle combination. The boundary conditions are applied as shown in Figure (\ref{fig:AlignedRamp_setup}). We adopt three grid resolutions similar to the aligned oblique shock case.

In this subsection, we examine the scenario where the incoming flow, outflow, and shock are all aligned with the grid. To achieve this, we use a computational domain as illustrated in Figure (\ref{fig:AlignedRamp_setup}) for a flow over a ramp test case. The computational domain comprises two parallelograms, ABEF and BCDE.

The parallelogram ABEF is designed such that the sides AB and EF are parallel to the x-axis, while sides BE and AF are inclined at an angle $\beta$ (shock angle) to the positive x-axis. Similarly, the parallelogram BCDE is constructed with sides BC and DE inclined at an angle $\theta$ (turn angle) to the positive x-axis, and side CD parallel to side BE. Various combinations of shock and turn angles result in different computational domains. This construction aligns the shock but results in a skewed grid. However, the focus of this paper is not on the skewness of the grid and the effects of skewness are not studied in this investigation.

The computational domain is initialized with the exact solution for the respective inlet Mach number, shock angle, and turn angle combination. Boundary conditions are applied as depicted in Figure (\ref{fig:AlignedRamp_setup}). We employ three grid resolutions similar to those used in the aligned oblique shock case. Since the shock is aligned to the grid, pre-labelling the troubled cells is similar to the aligned oblique shock case.

\begin{figure}[H]
\centering
\includestandalone[width=0.8\textwidth]{./4-Main/AlignedRamp/AlignedRamp_setup}\label{fig:AlignedRamp_setup}\\
\caption{Schematic representation for the flow over a ramp where the shock is aligned to the grid, illustrating the varying geometric and flow conditions, and boundary conditions. (not drawn to scale).}
\label{fig:AlignedRamp_setup}
\end{figure}

Density profiles of the cells along the center stream line for three different shock angles with an inlet Mach number of 3, using the medium grid are shown in Figure (\ref{fig:AR_density_PreAndPost1}) for configurations with a single troubled-cell either in pre- or post-shock region. Figure (\ref{fig:AR_density_2and3}) illustrates the density profiles for configurations with at least two troubled cells in both the pre- and post-shock regions.

\begin{figure}[H]
\centering
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR30_density_pre1}\label{fig:AR30_density_pre1}}
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR30_density_post1}\label{fig:AR30_density_post1}}\\
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR40_density_pre1}\label{fig:AR40_density_pre1}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR40_density_post1}\label{fig:AR40_density_post1}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR50_density_pre1}\label{fig:AR50_density_pre1}}
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR50_density_post1}\label{fig:AR50_density_post1}}
\caption{Flow over a ramp with inlet Mach 3. Density profiles along the center stream line for three different shock angles on the medium grid. Top row (a, b): \ang{30}. Middle row (c, d): \ang{40}. Bottom row (e, f): \ang{50}. Left column (a, c, e): configurations with a single troubled-cell in the pre-shock. Right column (b, d, f): configurations with a single troubled-cell in the post-shock.}
\label{fig:AR_density_PreAndPost1}
\end{figure}

\begin{figure}[H]
\centering
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR30_density_post2}\label{fig:AR30_density_post2}}
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR30_density_post3}\label{fig:AR30_density_post3}}\\
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR40_density_post2}\label{fig:AR40_density_post2}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR40_density_post3}\label{fig:AR40_density_post3}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR50_density_post2}\label{fig:AR50_density_post2}}
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/AR50_density_post3}\label{fig:AR50_density_post3}}
\caption{Flow over a ramp with inlet Mach 3. Density profiles along the center stream line for three different shock angles on the medium grid. Top row (a, b): \ang{30}. Middle row (c, d): \ang{40}. Bottom row (e, f): \ang{50}. Left column (a, c, e): configurations with two troubled-cells in the post-shock. Right column (b, d, f): configurations with two troubled-cells in the post-shock.}
\label{fig:AR_density_2and3}
\end{figure}

\begin{figure}[H]
\centering
\includestandalone[width=0.25\textwidth]{./4-Main/AlignedRamp/SameMach/legend}\\[-5ex]
\includegraphics[width=\textwidth]{./4-Main/AlignedRamp/SameMach/Density}\label{fig:SameMachDensity}
\caption{Flow over a ramp with inlet Mach 3. $\mu$ for three different shock angles across all configurations, including the limiting-everywhere case. ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:AR_SameMach_TvLinfDiff}
\end{figure}

\begin{figure}[H]
\centering
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/30_post2}\label{fig:AR_RN_30_post2}}
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/30_post3}\label{fig:AR_RN_30_post3}}\\
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/40_post2}\label{fig:AR_RN_40_post2}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/40_post3}\label{fig:AR_RN_40_post3}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/50_post2}\label{fig:AR_RN_50_post2}}
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/AlignedRamp/50_post3}\label{fig:AR_RN_50_post3}}
\caption{Flow over a ramp with inlet Mach 3. The convergence history of the residual norm as a function of number of iterations. Top row (a, b): \ang{30}. Middle row (c, d): \ang{40}. Bottom row (e, f): \ang{50}. Left column (a, c, e): configurations with two troubled-cells in the post-shock. Right column (b, d, f): configurations with two troubled-cells in the post-shock.}
\label{fig:AlignedOS_M3_RN_Main}
\end{figure}


\begin{figure}[H]
\centering
\includestandalone[width=0.3\textwidth]{./4-Main/AlignedRamp/SameAngle/legend}\\[-5ex]
\subfloat[\ang{30}]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignedRamp/SameAngle/Density2_30}\label{fig:SameAngleDensity_30}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignedRamp/SameAngle/Density2_40}\label{fig:SameAngleDensity_40}}\\[-2ex]
\subfloat[\ang{50}]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignedRamp/SameAngle/Density2_50}\label{fig:SameAngleDensity_50}}
\caption{Flow over a ramp. $\mu$ for three different upstream Mach numbers for a given shock angle. For upstream Mach numbers $M_{PR_1}$, $M_{PR_2}$, and $M_{PR_3}$ (in ascending order), refer Table (\ref{tab:AOS_SameAngle}). ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:AR_SameAngle_TvLinfDiff}
\end{figure}

\begin{figure}[H]
\centering
\includestandalone[width=0.3\textwidth]{./4-Main/AlignedRamp/SamePR/legend}\\[-5ex]
\subfloat[$PR_1$]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignedRamp/SamePR/Density2_PR1}\label{fig:SamePRDensity_PR1}}
\subfloat[$PR_2$]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignedRamp/SamePR/Density2_PR2}\label{fig:SamePRDensity_PR2}}\\[-2ex]
\subfloat[$PR_3$]{\includegraphics[width=0.5\textwidth]{./4-Main/AlignedRamp/SamePR/Density2_PR3}\label{fig:SamePRDensity_PR3}}
\caption{Flow over a ramp. $\mu$ for three different upstream Mach number and shock angle combinations for a given pressure ratio. For pressure ratios $PR_1$, $PR_2$, and $PR_3$ (in ascending order), refer Table (\ref{tab:AOS_SameAngle}). ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:AR_SamePR_TvLinfDiff}
\end{figure}


==> 6-Results/NonAlignOS/NonAlignOS.tex <==
\subsection{Non-Aligned Oblique Shock}

% \input{./4-Main/Label_TC_Methods/NonAlign/NonAlignedShocks.tex}

We solve the two-dimensional Euler equations (\ref{eq:2d_euler}) for the test setup shown in Figure (\ref{fig:NonAlignOS_setup}), considering three different shock angles for a given upstream Mach number in the first case. The computational domain is initialised with the exact solution corresponding to an upstream Mach number of $3$ and the shock angle of interest. The limiter is applied only to troubled-cells, which are identified by tracing the parallel lines using the line tracing algorithm given in Algorithm (\ref{alg:LTA}) for various configurations shown in Figure (\ref{fig:Method3_cases}).

Similar to the case of aligned oblique shocks, we investigated two different cases for non-aligned oblique shocks: one with various oblique shock angles for a given upstream Mach number, and the other with various upstream Mach numbers for a given oblique shock angle. Additionally, we investigated cases where the shock is fixed at a particular angle with respect to the grid by changing the upstream flow angles for different combinations of upstream Mach numbers and shock angles.

Density profiles of the cells just above the line $y = 0.5$ for three different oblique shock angles using the medium grid are shown in Figure (\ref{fig:NAOS_density_PreAndPost1}). These solutions are obtained by limiting only the troubled cells, which are identified by tracing a single parallel line to the shock line either in pre- or post-shock region. Similar to the case of aligned oblique shocks, solutions of these configurations exhibit undershoots and overshoots in the pre- and post-shock regions, respectively. These figures suggest that adding extra troubled-cells in the post-shock region, while keeping the troubled-cells in the pre-shock region fixed, does not significantly affect the solution in pre-shock region. Similarly, adding extra troubled-cells in the pre-shock region, while keeping the troubled-cells in the post-shock region fixed, does not significantly affect the solution in the post-shock region.

\begin{figure}[H]
\centering
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA30_density_pre1}\label{fig:NA30_density_pre1}}
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA30_density_post1}\label{fig:NA30_density_post1}}\\
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA40_density_pre1}\label{fig:NA40_density_pre1}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA40_density_post1}\label{fig:NA40_density_post1}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA50_density_pre1}\label{fig:NA50_density_pre1}}
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA50_density_post1}\label{fig:NA50_density_post1}}
\caption{Non-aligned oblique shock with upstream Mach number 3. Density profiles along the line $y = 0.5$ for three different shock angles on the medium grid. Top row (a, b): \ang{30}. Middle row (c, d): \ang{40}. Bottom row (e, f): \ang{50}. Left column (a, c, e): configurations with a single parallel line in the pre-shock. Right column (b, d, f): configurations with a single parallel line in the post-shock.}
\label{fig:NAOS_density_PreAndPost1}
\end{figure}

Density profiles of the cells along the same line are shown in Figure (\ref{fig:NAOS_density_Post2And3}) for configurations `22', `32', and `42' on the left side and configurations `23', `33', and `43' on the right side.
There are no significant overshoots or undershoots in the solutions of these configurations compared to the configurations with a single parallel line either in the pre- or post-shock region. However, slight undershoots and overshoots are present for configurations with two parallel lines in the pre-shock region or two parallel lines in the post-shock region.

From Figures (\ref{fig:NAOS_density_PreAndPost1}) and (\ref{fig:NAOS_density_Post2And3}), we observe that as the shock angle increases, oscillations in the pre-shock region also increase. Conversely, oscillations in the post-shock region decrease. This suggests that a greater number of troubled cells is needed in the pre-shock region for higher shock angles, while a greater number of troubled cells is required in the post-shock region for smaller shock angles.

\begin{figure}[H]
\centering
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA30_density_post2}\label{fig:NA30_density_post2}}
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA30_density_post3}\label{fig:NA30_density_post3}}\\
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA40_density_post2}\label{fig:NA40_density_post2}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA40_density_post3}\label{fig:NA40_density_post3}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA50_density_post2}\label{fig:NA50_density_post2}}
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/NA50_density_post3}\label{fig:NA50_density_post3}}
\caption{Non-aligned oblique shock with upstream Mach number 3. Density profiles along the line $y = 0.5$ for three different shock angles on the medium grid. Top row (a, b): \ang{30}. Middle row (c, d): \ang{40}. Bottom row (e, f): \ang{50}. Left column (a, c, e): configurations with two parallel lines in the post-shock. Right column (b, d, f): configurations with three parallel lines in the post-shock.}
\label{fig:NAOS_density_Post2And3}
\end{figure}

Figure (\ref{fig:NAOS_SameMach_TvLinfDiff}) further confirms these observations by showing the differences ($\mu$) between the total variation and $L_{\infty}$ norm of the error in density for three different shock angles for a given upstream Mach number across all configurations, including limiting everywhere case.

For configurations with a single parallel line either in the pre- or post-shock region, the difference is significantly higher compared to other configurations, indicating the presence of significant oscillations in the solution, as shown in Figure (\ref{fig:NAOS_density_PreAndPost1}). For all other configurations, with at least two parallel lines in both the pre- and post-shock regions, the difference is of the order $10 ^{-2}$ or smaller. From Figure (\ref{fig:NAOS_SameMach_TvLinfDiff}), it can also be observed that adding extra troubled-cells in the pre-shock region does not significantly affect the solution for smaller shock angles, while it significantly improves the solution for higher shock angles. Conversely, adding extra troubled-cells in the post-shock region improves the solution for smaller shock angles, while it does not affect the solution for higher shock angles.

\begin{figure}[H]
\centering
\includestandalone[width=0.25\textwidth]{./4-Main/NonAlignOS/M3/SameMach/legend}\\[-5ex]
\includegraphics[width=\textwidth]{./4-Main/NonAlignOS/M3/SameMach/Density}\label{fig:NAOS_SameMachDensity}
\caption{Non-aligned oblique shock with upstream Mach number 3: $\mu$ for three different shock angles across all configurations including the limiting everywhere case. ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:NAOS_SameMach_TvLinfDiff}
\end{figure}

From here on, we present the results only for configurations with at least two parallel lines both in the pre- and post-shock regions for all other test cases involving non-aligned shocks. The convergence history of the residual norm $RN$ (Eq. \ref{eq:RN}) versus number of iterations is plotted in Figure (\ref{fig:NonAlignedOS_M3_RN}) for three different oblique shock angles and configurations `22', `23', `32', and `23'. It can be observed that the solution fully converges (i.e., $RN < 10^{-14}$) to steady-state solution in nearly the same number of iterations for all these configurations particularly for the \ang{50} shock angle, which is significantly better than the limiting everywhere approach. However, for \ang{30} and \ang{40} shock angles, residual norm fully converged only for the configurations with two parallel lines in post-shock region, while the configurations with more than two parallel lines in the post-shock region, residual norm converged to same level as limiting everywhere case. Overall, limiting only the neighbourhood of the shock significantly improves the convergence compared to the limiting everywhere case.

\begin{figure}[H]
\centering
\subfloat[\ang{30}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/residuenorm_30}\label{fig:NAOS_RN_30}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/residuenorm_40}\label{fig:NAOS_RN_40}}\\
\subfloat[\ang{50}]{\includegraphics[width=0.5\linewidth]{./4-Main/NonAlignOS/M3/residuenorm_50}\label{fig:NAOS_RN_50}}
\caption{Non-aligned oblique shock with inlet Mach 3. The convergence history of the residual norm as a function of number of iterations for configurations `22', `23', `32', and `33', and for limiting everywhere case.}
\label{fig:NonAlignedOS_M3_RN}
\end{figure}

For the second case, we varied the Mach numbers for a given shock angle. We selected the same upstream Mach numbers as we did for the aligned shock cases, as shown in Table (\ref{tab:AOS_SameAngle}). Results are presented for both cases: one with respect to shock angle, and the other with respect to pressure ratio in Figures (\ref{fig:NAOS_SameAngle_TvLinfDiff}) and (\ref{fig:NAOS_SamePR_TvLinfDiff}), respectively. These results indicate the same observations made earlier, that adding extra troubled cells in the pre-shock region improves the solution for higher shock angles, and adding extra troubled cells in the post-shock region improves the solution for smaller shock angles.

\begin{figure}[H]
\centering
\includestandalone[width=0.3\textwidth]{./4-Main/AlignOS/M3/SameAngle/legend}\\[-2ex]
\subfloat[\ang{30}]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/M3/SameAngle/Density2_30}\label{fig:NAOS_SameAngleDensity_30}}
\subfloat[\ang{40}]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/M3/SameAngle/Density2_40}\label{fig:NAOS_SameAngleDensity_40}}\\[-2ex]
\subfloat[\ang{50}]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/M3/SameAngle/Density2_50}\label{fig:NAOS_SameAngleDensity_50}}
\caption{Non-aligned oblique shock: $\mu$ for three different upstream Mach numbers for a given shock angle. For upstream Mach numbers $M_{PR_1}$, $M_{PR_2}$, and $M_{PR_3}$ (in ascending order), refer Table (\ref{tab:AOS_SameAngle}). ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:NAOS_SameAngle_TvLinfDiff}
\end{figure}

\begin{figure}[H]
\centering
\includestandalone[width=0.3\textwidth]{./4-Main/AlignOS/M3/SamePR/legend}\\[-2ex]
\subfloat[$PR_1$]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/M3/SamePR/Density2_PR1}\label{fig:NAOS_SamePRDensity_PR1}}
\subfloat[$PR_2$]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/M3/SamePR/Density2_PR2}\label{fig:NAOS_SamePRDensity_PR2}}\\[-2ex]
\subfloat[$PR_3$]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/M3/SamePR/Density2_PR3}\label{fig:NAOS_SamePRDensity_PR3}}
\caption{Non-aligned oblique shock: $\mu$ for three different upstream Mach number and shock angle combinations for a given pressure ratio. For pressure ratios $PR_1$, $PR_2$, and $PR_3$ (in ascending order), refer Table (\ref{tab:AOS_SameAngle}). ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:NAOS_SamePR_TvLinfDiff}
\end{figure}

For the third case, we fixed the shock at a particular angle with respect to the grid to determine the dependence of number of troubled-cells on whether it is the actual shock angle or the shock angle with respect to the grid. We examined two different scenarios: one where the upstream Mach number is kept constant, and the other where the pressure ratio across the shock is kept constant. Tables (\ref{tab:FixedMisAlignment_SameMach}) and (\ref{tab:FixedMisAlignment_SamePR}) present the upstream flow angles and Mach numbers for three different shock angles for a fixed misalignment of the shock with respect to the grid.

\begin{table}[H]
\centering
\caption{For a fixed misalignment with respect to the grid, different shock angles and the corresponding upstream flow angles.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c c c c c}
\toprule
 \makecell{Fixed misalignment\\w.r.t grid} & Mach number & \makecell{Upstream flow\\angle(in degrees)} & \makecell{Actual shock \\angle (in degrees)} & \makecell{Downstream flow \\angle (in degrees)}\\
\midrule
\multirow{3}{*}{\ang{30}} & 3 & 0 & 30 & 12.77\\
& 3 & -10 & 40 & 11.84\\
& 3 & -20 & 50 & 8.86\\
\midrule
\multirow{3}{*}{\ang{40}} & 3 & 10 & 30 & 22.77\\
& 3 & 0 & 40 & 21.84\\
& 3 & -10 & 50 & 18.86\\
\midrule
\multirow{3}{*}{\ang{50}} & 3 & 20 & 30 & 32.77 \\
& 3 & 10 & 40 & 31.84 \\
& 3 & 0 & 50 & 28.86 \\
\bottomrule
\end{tabular}%
}
\label{tab:FixedMisAlignment_SameMach}
\end{table}

\begin{table}[H]
\centering
\caption{For a fixed misalignment with respect to the grid, different shock angles and the upstream Mach number combinations such that the pressure ratio across the shock is same.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c c c c c}
\toprule
 \makecell{Fixed misalignment\\w.r.t grid} & Mach number & \makecell{Upstream flow\\angle(in degrees)} & \makecell{Actual shock \\angle (in degrees)} & \makecell{Downstream flow \\angle (in degrees)}\\
\midrule
\multirow{3}{*}{\ang{30}} & 3 & 0 & 30 & 12.77\\
& 2.33358574 & -10 & 40 & 5.74\\
& 1.958110935 & -20 & 50 & -2.72\\
\midrule
\multirow{3}{*}{\ang{40}} & 3.85672566 & 10 & 30 & 27.28\\
& 3 & 0 & 40 & 21.84\\
& 2.517298895 & -10 & 50 & 15.02\\
\midrule
\multirow{3}{*}{\ang{50}} & 4.59626666 & 20 & 30 & 39.39 \\
& 3.57526078 & 10 & 40 & 34.77 \\
& 3 & 0 & 50 & 28.86 \\
\bottomrule
\end{tabular}%
}
\label{tab:FixedMisAlignment_SamePR}
\end{table}

Results are presented in Figures (\ref{fig:FMA_SameMach_TvLinfDiff}) and (\ref{fig:FMA_SamePR_TvLinfDiff}) for the same upstream Mach number case and the same pressure ratio case, respectively. By examining the results of the \ang{50} shock misalignment with respect to the grid in Figures (\ref{fig:FMA_SameMach_50}) and (\ref{fig:FMA_SamePR_50}), we observe that for all three shock angles, the effect of the troubled cells is same i.e., adding extra troubled-cells in the pre-shock region improves the solution, but not in the post-shock region, although this is quite the opposite for smaller shock angles, as seen earlier. This concludes that the dependence of number of troubled-cells is actually on the shock angle with respect to the grid rather than the actual shock angle.

\begin{figure}[H]
\centering
\includestandalone[width=0.3\textwidth]{./4-Main/AlignOS/M3/SamePR/legend}\\[-5ex]
\subfloat[\ang{30} fixed misalignment wrt grid]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/FixedMisAlignment/SameMach/Density2_30}\label{fig:FMA_SameMach_30}}
\subfloat[\ang{40} fixed misalignment wrt grid]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/FixedMisAlignment/SameMach/Density2_40}\label{fig:FMA_SameMach_40}}\\[-2ex]
\subfloat[\ang{50} fixed misalignment wrt grid]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/FixedMisAlignment/SameMach/Density2_50}\label{fig:FMA_SameMach_50}}
\caption{Fixed misalignment of the shock with respect to the grid: $\mu$ for three different shock angles for a given fixed misalignment of the shock with respect to the grid given in Table (\ref{tab:FixedMisAlignment_SameMach}). ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:FMA_SameMach_TvLinfDiff}
\end{figure}

\begin{figure}[H]
\centering
\includestandalone[width=0.3\textwidth]{./4-Main/AlignOS/M3/SamePR/legend}\\[-5ex]
\subfloat[\ang{30} fixed misalignment wrt grid]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/FixedMisAlignment/SamePR/Density2_30}\label{fig:FMA_SamePR_30}}
\subfloat[\ang{40} fixed misalignment wrt grid]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/FixedMisAlignment/SamePR/Density2_40}\label{fig:FMA_SamePR_40}}\\[-2ex]
\subfloat[\ang{50} fixed misalignment wrt grid]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/FixedMisAlignment/SamePR/Density2_50}\label{fig:FMA_SamePR_50}}
\caption{Fixed misalignment of the shock with respect to the grid: $\mu$ for three different shock angles for a given fixed misalignment of the shock with respect to the grid given in Table (\ref{tab:FixedMisAlignment_SamePR}). ($\mu = \text{TV} - L_{\infty}$)}
\label{fig:FMA_SamePR_TvLinfDiff}
\end{figure}

Notably, for the \ang{30} misalignment with respect to the grid, the scenarios with the upstream Mach number $M = 2.33358574$ for a \ang{40} shock angle, and both the upstream numbers for a \ang{50} shock angle, the solution exhibits significant oscillations in the post-shock region, even for the approach of limiting everywhere. The density profiles for these cases are shown in Figure (\ref{fig:G30_A4050}).

\begin{figure}[H]
\centering
\subfloat[\ang{40}, $M = 2.33358574$]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/FixedMisAlignment/G30_A40_M23_density}\label{fig:G30_A40_M23}}
\subfloat[\ang{50}, $M=3$]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/FixedMisAlignment/G30_A50_M3_density}\label{fig:G30_A50_M3}}\\
\subfloat[\ang{50}, $M=1.958110935$]{\includegraphics[width=0.5\textwidth]{./4-Main/NonAlignOS/FixedMisAlignment/G30_A50_M19_density}\label{fig:G30_A50_M19}}
\caption{\ang{30} misalignment of the shock with respect to the grid: Density profiles along the line $y = 0.5$ for three different combinations of upstream Mach numbers and shock angles on the medium grid.}
\label{fig:G30_A4050}
\end{figure}

